GradInit: Learning to Initialize Neural Networks for Stable and Efficient Training

Innovations in neural architectures have fostered significant breakthroughs in language modeling and computer vision. Unfortunately, novel architectures often result in challenging hyper-parameter choices and training instability if the network parameters are not properly initialized. A number of architecture-specific initialization schemes have been proposed, but these schemes are not always portable to new architectures. This paper presents GradInit, an automated and architecture agnostic method for initializing neural networks. GradInit is based on a simple heuristic; the norm of each network layer is adjusted so that a single step of SGD or Adam with prescribed hyperparameters results in the smallest possible loss value. This adjustment is done by introducing a scalar multiplier variable in front of each parameter block, and then optimizing these variables using a simple numerical scheme. GradInit accelerates the convergence and test performance of many convolutional architectures, both with or without skip connections, and even without normalization layers. It also improves the stability of the original Transformer architecture for machine translation, enabling training it without learning rate warmup using either Adam or SGD under a wide range of learning rates and momentum coefficients. Code is available at https://github.com/zhuchen03/gradinit.

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{} One limitation of our current work is we have not checked whether GradInit can improve the training of models from other domains such as speech.
  \item Did you discuss any potential negative societal impacts of your work?
   \answerNA{} % \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
   \answerNA{} % \answerYes{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tables/cifar10_all.tex <==

\begin{table}[htbp!]
% \resizebox{\linewidth}{!}{%
\begin{tabular}{clcc}
\toprule 
\begin{tabular}[c]{@{}c@{}}Model \\ (\#Params)\end{tabular}                             & Method     & $Acc_0$       & $Acc_{best}$    \\
\midrule 
 \multicolumn{4}{l}{On CIFAR-10} \\
\midrule 
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}VGG-19 \\ w/o BN \\ (20.03 M)\end{tabular}}  & Kaiming  & 29.14 $\pm$ 1.49 & 94.48 $\pm$ 0.09 \\
                                                                                        & MetaInit & \bf{30.48 $\pm$ 0.88} & 94.62 $\pm$ 0.06 \\
                                                                                        & GradInit & 29.25 $\pm$ 0.55 & \bf{94.71 $\pm$ 0.02} \\
\midrule 
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}VGG-19 \\ w/ BN \\ (20.04M)\end{tabular}}    & Kaiming  & 12.57 $\pm$ 0.59 & 94.41 $\pm$ 0.09 \\
                                                                                        & MetaInit & 35.09 $\pm$ 0.58 &  94.64 $\pm$ 0.07 \\
                                                                                        & GradInit & \bf{47.79 $\pm$ 1.79} & \bf{95.13 $\pm$ 0.07} \\
\midrule 
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}ResNet-110\\ w/o BN\\ (1.72M)\end{tabular}}  & Kaiming  & 16.05 $\pm$ 2.05 & 94.22 $\pm$ 0.09 \\
                                                                                        & MetaInit & 14.55 $\pm$ 2.19 &  94.19 $\pm$ 0.11 \\
                                                                                        & GradInit & \bf{36.21 $\pm$ 0.78} & \bf{94.60 $\pm$ 0.13} \\
\midrule 
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}ResNet-110\\ w/ BN\\ (1.73M)\end{tabular}}   & Kaiming  & 23.15  $\pm$ 0.93 & 94.98  $\pm$ 0.16 \\
                                                                                        & MetaInit  &  29.00 $\pm$ 1.45  &  94.76 $\pm$ 0.08  \\
                                                                                        & GradInit  & \bf{38.19 $\pm$ 0.85} & \bf{95.38 $\pm$ 0.05} \\
\midrule 
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}WRN-28-10\\ w/ BN\\ (36.49M)\end{tabular}}   & Kaiming  & 43.10 $\pm$ 2.72 &  97.22 $\pm$ 0.05 \\
                                                                                        & MetaInit$^*$  &  -  &  97.1   \\
                                                                                        & GradInit  & \bf{46.28 $\pm$ 0.44} & \bf{97.29 $\pm$ 0.07} \\
\midrule 
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}FixUpResNet\\ (1.72M)\end{tabular}}          & FixUp     & \bf{38.17 $\pm$ 0.83} & \bf{95.38 $\pm$ 0.08} \\
                                                                                        & MetaInit  & 21.49 $\pm$ 0.60 &  95.00 $\pm$ 0.14  \\
                                                                                        & GradInit  & 35.62 $\pm$ 1.47  &  95.33 $\pm$ 0.03 \\
                                                                                        & GradInit$^{\dagger}$  & 34.97 $\pm$ 0.65  &  \bf{95.38 $\pm$ 0.06} \\
\midrule 
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}DenseNet-100\\ w/o BN\\ (0.75M)\end{tabular}} & Kaiming$^{\ddagger}$  &  35.54 $\pm$ 0.58 & 93.97 $\pm$ 0.09 \\
                                                                                        & MetaInit &       35.11 $\pm$ 0.20 & 94.43 $\pm$ 0.08 \\
                                                                                        & GradInit  &     \bf{37.19 $\pm$ 1.05} & \bf{94.85 $\pm$ 0.06} \\
\midrule 
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}DenseNet-100 \\ w/ BN\\ (0.77M)\end{tabular}} & Kaiming  &    51.23 $\pm$ 1.46 & 95.46 $\pm$ 0.06 \\
                                                                                        & MetaInit &      46.67 $\pm$ 4.00 & 95.47 $\pm$ 0.08 \\
                                                                                        & GradInit  &     \bf{52.80 $\pm$ 0.79} & \bf{95.50 $\pm$ 0.08} \\
\midrule 
 \multicolumn{4}{l}{On ImageNet} \\
\midrule 
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}ResNet-50\\ w/ BN\\ (25.6M)\end{tabular}} & Kaiming  &   14.61 $\pm$ 0.24    & 75.91  $\pm$ 0.09 \\
                                                                              & MetaInit$^{*}$  &   -   &  75.4  \\
                                                                              & GradInit  &    \bf{19.20 $\pm$ 0.77}    & \textbf{76.21 $\pm$ 0.08}  \\
\bottomrule
\end{tabular}
% }
\caption{\footnotesize First epoch ($Acc_0$) and best test accuracy over all epochs ($Acc_{best}$) for models on CIFAR-10 and ImageNet. We report the mean and its standard error of the top-1 test accuracy in 4 experiments with different random seeds. Best results in each group are in bold. $\dagger$ Achieved by using $\tilde{S}\cup S=\emptyset$. $^\ddagger$ For DenseNet-100 without BN, we found MetaInit and GradInit to perform better when gradient clipping is not applied. However, Kaiming's initialization will not converge without gradient clipping, so we applied a gradient clipping of 1 to this setting. $^{*}$The result of MetaInit are taken from~\cite{dauphin2019metainit}. They use the variant of ResNet without BN from~\cite{zhang2019fixup}, and replaced the ReLU activations with Swish~\citep{ramachandran2017searching}, which is not directly comparable with our BN version, but we keep it here for convenience of reference.}
\zc{TODO: list resutls of second-epoch accuracy.}

\zc{Waiting: results for wrn-40-10: first epoch accuracy do not seem really better than training one additional epoch. What happens when training finishes? Some benefits from a better initialization? }
% \zheng{Maybe add row index number in this table? This table is too big and hard to track}
% \zc{Do it later. }
\label{tab:image_all}

\end{table}
